Active Self-Training for Weakly Supervised 3D Scene Semantic Segmentation

Since the preparation of labeled data for training semantic segmentation networks of point clouds is a time-consuming process, weakly supervised approaches have been introduced to learn from only a small fraction of data. These methods are typically based on learning with contrastive losses while automatically deriving per-point pseudo-labels from a sparse set of user-annotated labels. In this paper, our key observation is that the selection of what samples to annotate is as important as how these samples are used for training. Thus, we introduce a method for weakly supervised segmentation of 3D scenes that combines self-training with active learning. The active learning selects points for annotation that likely result in performance improvements to the trained model, while the self-training makes efficient use of the user-provided labels for learning the model. We demonstrate that our approach leads to an effective method that provides improvements in scene segmentation over previous works and baselines, while requiring only a small number of user annotations.

==> figures/tab_sup_percategory_s3dis.tex <==
%\begin{sidewaystable}[t!]
%	\scriptsize\addtolength{\tabcolsep}{-4pt}
%		\begin{center}
	%		\caption{Per-category performance of our method (ActiveST) and other weakly supervised methods on Scannet-v2 data-efficient benchmark (20 labelled points per scene for training).}
	%			\begin{tabular}{ c | c | c c c c c c c c c c c c c c c c c c c c c} \toprule  
		%                
		%            % 	Method  & mIoU & bathtub & bed & booksh. & cabinet & chair & counter & curtain & desk & door & floor & otherfur. & picture & refrigerator & shower. & sink & sofa & table & toilet & wall & window \\ \midrule 
		%            Method  & mIoU & bath. & bed & book. & cabi. & chai. & coun. & curt. & desk & door & flor. & otfr. & pict. & refri. & show. & sink & sofa & tabl. & toil. & wall & wind. \\ \midrule 
		%
		%				CSC~\cite{hou2021exploring} & 53.1 & 65.9	&63.8	&57.8	&41.7	&77.5	&25.4	&53.7	&39.6	&43.9&	93.9	&28.4	&8.3	&41.4	&59.9	&48.8	&69.8	&44.4	&78.5	&74.7	&44.0 \\ 
		%				PointContrast~\cite{xie2020} & 55.0 & 73.5&	67.6&	60.1&	47.5&	79.4&	28.8	&62.1&	37.8&	43.0&	94.0&	30.3&	8.9&	37.9&	58.0&	53.1&	68.9&	42.2&	85.2&	75.8&	46.8 \\
		%                1T1C~\cite{liu2021one} & 59.4 & 75.6&	72.2&	49.4&	54.6&	79.5&	37.1&	72.5&	55.9&	48.8&	95.7&	36.7&	\bf{26.1}&	54.7&	57.5&	22.5&	67.1&	54.3&	90.4&	82.6&	55.7 \\ \midrule
		%				ActiveST(Ours) & \bf{70.3} & \bf{97.7}&	\bf{77.6}&	\bf{65.7}&	\bf{70.7}&	\bf{87.4}&	\bf{54.1}&	\bf{74.4}&	\bf{60.5}&	\bf{61.0}&	\bf{96.8}&	\bf{44.2}&	12.6&	\bf{70.5}&	\bf{78.5}&	\bf{74.2}&	\bf{79.1}&	\bf{58.6}&	\bf{94.0}&	\bf{83.9}&	\bf{64.5} \\ \bottomrule 
		%			\end{tabular}
	%		\end{center}
%	\label{tab:sup_percategory}
%\end{sidewaystable}
\begin{table*}[t!]
	\caption{\blu{Per-category performance of our method on the S3DIS data-efficient benchmark (20 labeled points per scene for training). ``BS`` refers to the baseline which directly sample 20 labeled points per scene for training, ``ST`` denotes using self-training approach to generate the pseudo label to train the network, and ``AL`` denotes using active learning approach to iteratively select the labeld points to train the network.}}
	\label{tab:sup_percategory_s3dis}
	% 	\scriptsize\addtolength{\tabcolsep}{-4pt}
%	\scriptsize\addtolength{\tabcolsep}{-4.3pt}
	\scriptsize\addtolength{\tabcolsep}{-0.6pt}
	\begin{center}
		\begin{tabular}{ c | c | c c c c c c c c c c c c c} \toprule  
			
			Method  & mIoU & ceiling & floor & beam & column & beam & window & door & table & chair & bookcase & sofa & board & clutter \\ \midrule 
			
			BS & 40.5 & 88.9 & 92.6 & 72.9 & 5.3 & 0.0 & 37.3 & 44.2 & 44.0 & 47.0 & 48.1 & 3.1 & 10.1 & 32.9 \\
			ST & 47.2 & 90.1 & 93.0 & 73.2 & 5.1 & 0.0 & 38.3 & 56.0 & 61.5 & 74.8 & 63.1 & 2.0 & 14.1 & 43.0 \\
			AL & 51.8 & 88.1 & 93.6 & \bf{75.4} & 16.1 & 0.0 & \bf{40.3} & 46.7 & 63.3 & 75.6 & 62.2 & 13.6 & \bf{53.2} &  45.4 \\ \midrule
			Ours & \bf{56.6} & \bf{90.2} & \bf{93.9} &  \bf{75.4} & \bf{20.6} &	0.0 & 39.3 & \bf{62.3} & \bf{69.2} & \bf{81.9} & \bf{69.7} & \bf{58.2} & 25.2 & \bf{49.8} \\ \bottomrule 
		\end{tabular}
	\end{center}
\end{table*}

